Tactile-WAM: Touch-Aware World Action Model with Tactile Asymmetric Attention

World Action Models (WAMs) jointly predict future visual observations and actions, but visual futures alone often miss slip, jamming, contact-direction changes, and subtle misalign- ment in contact-rich manipulation. Tactile signals reveal these hidden physical states, yet naive tactile-token injection can disrupt visual dynamics modeling due to the limited scale of tactile data, a phenomenon we term tactile pollution. We in- troduce Tactile-WAM, which uses asymmetric attention to block video queries from tactile keys while preserving tac- tile access for action queries. A contact-change-aware bias further strengthens action attention to touch. Because tactile pixel changes do not reliably reflect contact changes, we derive Observed proxy changes drive the attention bias, while future- proxy supervision preserves action-relevant contact dynamics in predicted tactile representations. On ManiFeel, visual-path isolation reduces deviation from the RGB-only trajectory by 21.8% in MSE at the step-matched 20K checkpoint without a statistically detectable change in ground-truth video qual- ity. The full model improves average success from 15.6% to 32.7%, with VideoClean providing the largest gain. On five real-robot tasks, Tactile-WAM achieves 49.2% success.

==> sup_old_method.tex <==
This supplement gives additional model and evaluation details.
Both optical tactile streams are mosaicked and encoded by the same frozen Wan2.2 VAE used for RGB video~\citep{wan2025}; no separate tactile representation model is used.
The DiT jointly denoises video, tactile, and action variables.
During training, predicted clean tactile latents are decoded and supervised by a differentiable virtual-force proxy.
At inference, the attention bias comes only from observed tactile frames.
It does not use future tactile labels, decoded future force, or a previous denoising prediction.

\subsection{Training Computation}

For RGB video $o^v$ and left/right optical tactile videos $(o^{\tau,L},o^{\tau,R})$, the frozen Wan VAE encodes
\begin{equation}
z^v=E_{\rm Wan}(o^v),\qquad
z^\tau=E_{\rm Wan}(\mathcal M(o^{\tau,L},o^{\tau,R})),
\end{equation}
where $\mathcal M$ is horizontal mosaicking.
Tactile latent patches are projected into DiT registers, aligned to causal action blocks, and jointly denoised with video latents and actions.
For scheduler noise level $\sigma$, the predicted clean tactile future is reconstructed as
\begin{equation}
\widehat z_0^\tau=z_\sigma^\tau-\sigma v_\theta^\tau.
\end{equation}
The training-only physical path is:
\begin{enumerate}
    \item unpatchify the predicted tactile velocity and reconstruct $\widehat z_0^\tau$;
    \item prepend the observed tactile condition latent;
    \item decode through the frozen Wan VAE and map pixels to $[0,1]$;
    \item split the decoded mosaic back into left/right videos;
    \item estimate three virtual-force components from consecutive frames of each sensor and concatenate them into $\widehat F\in\mathbb R^{C\times8\times6}$;
    \item add Smooth-L1 supervision against cached force targets.
\end{enumerate}
The full model uses $\lambda_F=0.05$.
Gradients traverse the frozen decoder into the predicted tactile latents, but do not update Wan VAE parameters.
Virtual force is a deformation-derived proxy and is not reported as a calibrated wrench.

\subsection{Causal Routing Computation}

For training block anchor $u_c$, the cached routing input is
\begin{equation}
F_c^{\rm obs}=\Phi(o^\tau_{u_c-8},o^\tau_{u_c}).
\end{equation}
The first pair repeats the anchor and initializes the force input to zero.
Online inference instead uses the two most recent policy-call tactile observations and also returns zero on the initial call.
The force tensor is detached before routing.

Bias construction assigns one six-dimensional force value to the eight within-block transitions.
After norm, thresholding, temperature scaling, $\tanh$, temporal pooling, and spatial broadcasting, all tactile keys in a block receive the same value:
\begin{equation}
b_c=\operatorname{clip}\!\left(
\alpha\tanh\!\left(\frac{\operatorname{ReLU}(\|F_c^{\rm obs}\|_2-\theta)}{T}\right),
0,b_{\max}\right).
\end{equation}
Consequently, this mechanism is a blockwise tactile-modality gate, not spatial attention and not within-block temporal selection.
The additive term is applied only when the query is an action token and the key is a tactile token from the same block.

\videoclean{} is directional.
It removes tactile keys from the context available to video queries, while action queries keep tactile keys and tactile queries preserve their multimodal context.
The method therefore does not claim complete modality separation.

\subsection{Temporal and Action Settings}

The training cache indexes the released ManiFeel data at 10 fps~\citep{manifeel2025}.
The simulation environment runs physics at 60 Hz with control decimation four, yielding 15 Hz environment actions.
The model predicts 24 actions and executes eight before replanning.
Native six-dimensional task actions are right-zero-padded to the model's seven-dimensional interface and unpadded before environment execution; native seven-dimensional actions pass through unchanged.

\subsection{Ablation Configurations}

\begin{table}[t]
\centering
\small
\caption{Training configurations used in the component analysis.}
\label{tab:supp_profiles}
\begin{tabular}{lcccc}
\toprule
Configuration & Touch & Isolation & Bias & $\mathcal L_F$ \\
\midrule
RGB only & $\times$ & $\times$ & $\times$ & $\times$ \\
Tactile plain & \checkmark & $\times$ & $\times$ & $\times$ \\
Tactile isolation & \checkmark & \checkmark & $\times$ & $\times$ \\
Tactile full & \checkmark & \checkmark & \checkmark & \checkmark \\
\bottomrule
\end{tabular}
\end{table}

The configurations progressively add the Wan tactile stream, \videoclean{}, and the force-aware routing design used by the full \method{} model.
